SegMamba: Long-range Sequential Modeling Mamba For 3D Medical Image Segmentation

The Transformer architecture has shown a remarkable ability in modeling global relationships. However, it poses a significant computational challenge when processing high-dimensional medical images. This hinders its development and widespread adoption in this task. Mamba, as a State Space Model (SSM), recently emerged as a notable manner for long-range dependencies in sequential modeling, excelling in natural language processing filed with its remarkable memory efficiency and computational speed. Inspired by its success, we introduce SegMamba, a novel 3D medical image \textbf{Seg}mentation \textbf{Mamba} model, designed to effectively capture long-range dependencies within whole volume features at every scale. Our SegMamba, in contrast to Transformer-based methods, excels in whole volume feature modeling from a state space model standpoint, maintaining superior processing speed, even with volume features at a resolution of {$64\times 64\times 64$}. Comprehensive experiments on the BraTS2023 dataset demonstrate the effectiveness and efficiency of our SegMamba. The code for SegMamba is available at: https://github.com/ge-xing/SegMamba

==> 2_dataset.tex <==
\vspace{-1mm}
\section{Colorectal Cancer Segmentation Dataset (CRC-500)}
\vspace{-3mm}

\para{The Need for the CRC-500 Dataset}
Colorectal cancer (CRC) is the third most common cancer worldwide among men and women, the second leading cause of
death related to cancer, and the primary cause of death in gastrointestinal cancer~\cite{granados2017colorectal}.
%
% Using deep learning methods to detect the cancer region can assist doctors in making more accurate diagnoses.
%
However, as shown in Table \ref{tab:related_datasets}, the existing 3D colorectal cancer segmentation datasets are limited in size, and most of them are private.
%
% Moreover, only the MSD dataset is publicly available, but it lacks data on rectal cancer.
%
% To facilitate research in the 3D colorectal cancer segmentation field, 
% 
We contribute a new large-scale dataset (named CRC-500), which consists of 500 3D colorectal volumes with corresponding precise annotations from experts. 
%
Fig. \ref{fig:data_example} presents examples in 2D format from our proposed CRC-500 dataset. 
%The details of our CRC-500 will be discussed below.

\begin{figure*}[!t]
\centering
\includegraphics[width=0.8\textwidth]{figures/data_exsample.pdf}
\caption{
The data visualization for CRC-500 dataset.
} 
% \vspace{-3mm}
\label{fig:data_example}
\end{figure*}

\input{tables/related_dataset}

\para{Dataset Construct}
The CT scans were acquired from January 2008 to April 2020.
%
All sensitive patient information has been removed.
%
Each volume was annotated by a professional doctor and calibrated by another professional doctor.
%

% \noindent
\para{Dataset Analysis}
All the CT scans share the same in-plane dimension of $512\times 512$, and the dimension along the z-axis ranges from 94 to 238, with a median of 166.
%
The in-plane spacing ranges from $0.685\times 0.685$ mm to $0.925\times 0.925$ mm, with a median of $0.826\times 0.826$ mm, and the z-axis spacing is from 3.0 mm to 3.75 mm, with a median of 3.75 mm.




==> tables/brats23.tex <==
\begin{table*}[!t]
    \centering
    \caption{Quantitative comparison on BraTS2023 dataset, which contains four modalities and three segmentation targets (WT, TC, and ET). The bold value denotes the best performance.} 
    \label{tab:brats23}
    \renewcommand\arraystretch{1.2}
    % \setlength\tabcolsep{10pt}%调列距
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{c c c c c c c c c}
    \toprule

    \multirow{2}{*}{Methods} & \multicolumn{2}{c}{WT} & \multicolumn{2}{c}{TC}  & \multicolumn{2}{c}{ET}  & \multicolumn{2}{c}{Avg} \\
    
    & Dice $\uparrow$ & HD95 $\downarrow$ & Dice $\uparrow$ & HD95 $\downarrow$ & Dice $\uparrow$ & HD95 $\downarrow$ & Dice $\uparrow$ & HD95 $\downarrow$ \\
    \midrule
    
    SegresNet~\cite{myronenko20183d} & 92.02 & 4.07 & 89.10  & 4.08  & 83.66 & 3.88 & 88.26 & 4.01 \\

    UX-Net~\cite{lee20223d} & 93.13 & 4.56 & 90.03 &5.68 &	85.91 & 4.19  & 	89.69  & 4.81 \\
    MedNeXt~\cite{roy2023mednext} & 92.41  &4.98 & 	87.75  & 4.67  &	83.96  & 4.51  & 88.04 &4.72 \\
    \midrule

    UNETR~\cite{hatamizadeh2022unetr} & 92.19 & 6.17 & 	86.39  & 5.29  & 84.48  & 5.03 & 87.68  & 5.49 \\
    SwinUNETR~\cite{hatamizadeh2022swin} & 92.71  & 5.22 & 	87.79  & 4.42  & 	84.21  & 4.48 & 	88.23 & 4.70\\
    SwinUNETR-V2~\cite{he2023swinunetr} & 93.35 & 5.01 & 	89.65  & 4.41 & 	85.17 & 4.41  & 	89.39  & 4.51\\

    \midrule
    \rowcolor{gray!15} 
    Ours & \textbf{93.61} & \textbf{3.37 } & \textbf{92.65 } & \textbf{3.85 } & \textbf{87.71} & \textbf{3.48 } & 	\textbf{91.32 } & \textbf{3.56} \\
    
    \bottomrule
    \end{tabular}
    }
\end{table*}
